Augmented prediction of a true class for Positive Unlabeled data under selection bias

We introduce a new observational setting for Positive Unlabeled (PU) data where the observations at prediction time are also labeled. This occurs commonly in practice -- we argue that the additional information is important for prediction, and call this task "augmented PU prediction". We allow for labeling to be feature dependent. In such scenario, Bayes classifier and its risk is established and compared with a risk of a classifier which for unlabeled data is based only on predictors. We introduce several variants of the empirical Bayes rule in such scenario and investigate their performance. We emphasise dangers (and ease) of applying classical classification rule in the augmented PU scenario -- due to no preexisting studies, an unaware researcher is prone to skewing the obtained predictions. We conclude that the variant based on recently proposed variational autoencoder designed for PU scenario works on par or better than other considered variants and yields advantage over feature-only based methods in terms of accuracy for unlabeled samples.

==> standard-vae-pu/F1_score.tex <==
\begin{table}[tbp]
	\centering \scriptsize \renewcommand{\arraystretch}{1.2}
	\caption{F1 score values -- VAE-PU-Bayes (traditional PU setting)}
	\label{tab:F1_score}
\scalebox{0.63}{
	\begin{tabular}{llllllll}
		\toprule
		\textbf{c} & \textbf{Method} & \textbf{MNIST 3v5} & \textbf{MNIST OvE} & \textbf{CIFAR CT} & \textbf{CIFAR MA} & \textbf{STL MA} & \textbf{CDC Diabetes} \\
		\midrule
		\multirow{4}{*}{0.02} & VP &  \textbf{82.47 $\pm$ 0.75} &           74.40 $\pm$ 1.28 &           88.32 $\pm$ 0.51 &           88.91 $\pm$ 0.51 &           78.89 $\pm$ 0.53 &  \textbf{66.62 $\pm$ 0.20} \\
		     & VP-$A^3$ &           81.27 $\pm$ 0.63 &           76.97 $\pm$ 1.17 &           84.33 $\pm$ 0.94 &           88.96 $\pm$ 0.30 &           75.72 $\pm$ 0.52 &           65.53 $\pm$ 0.29 \\
		     & VP-IF &           81.56 $\pm$ 0.56 &  \textbf{77.17 $\pm$ 0.88} &           90.08 $\pm$ 1.14 &           87.59 $\pm$ 0.40 &           74.28 $\pm$ 0.93 &           66.51 $\pm$ 0.26 \\
		     & VP-B &           81.04 $\pm$ 0.69 &           73.07 $\pm$ 1.76 &  \textbf{91.75 $\pm$ 0.91} &  \textbf{92.11 $\pm$ 0.21} &  \textbf{80.59 $\pm$ 0.72} &           58.22 $\pm$ 1.07 \\
		\cline{1-8}
		\multirow{4}{*}{0.10} & VP &           86.41 $\pm$ 0.43 &           80.98 $\pm$ 0.63 &           91.63 $\pm$ 0.17 &           90.07 $\pm$ 0.32 &           83.49 $\pm$ 0.24 &           66.99 $\pm$ 0.18 \\
		     & VP-$A^3$ &           90.57 $\pm$ 0.27 &           83.95 $\pm$ 1.13 &           90.89 $\pm$ 0.39 &           90.81 $\pm$ 0.32 &           82.38 $\pm$ 0.45 &           66.39 $\pm$ 0.42 \\
		     & VP-IF &           90.79 $\pm$ 0.27 &           84.32 $\pm$ 1.08 &           92.46 $\pm$ 0.33 &           88.65 $\pm$ 0.55 &           82.22 $\pm$ 0.42 &  \textbf{67.28 $\pm$ 0.39} \\
		     & VP-B &  \textbf{91.46 $\pm$ 0.46} &  \textbf{86.30 $\pm$ 0.95} &  \textbf{93.72 $\pm$ 0.18} &  \textbf{93.01 $\pm$ 0.18} &  \textbf{85.72 $\pm$ 0.31} &           63.23 $\pm$ 0.71 \\
		\cline{1-8}
		\multirow{4}{*}{0.30} & VP &           88.79 $\pm$ 0.35 &           85.83 $\pm$ 0.22 &           93.11 $\pm$ 0.28 &           92.41 $\pm$ 0.14 &           86.16 $\pm$ 0.26 &           68.31 $\pm$ 0.19 \\
		     & VP-$A^3$ &           93.04 $\pm$ 0.20 &           90.65 $\pm$ 0.23 &           90.20 $\pm$ 0.66 &           91.97 $\pm$ 0.12 &           83.91 $\pm$ 0.35 &           70.66 $\pm$ 0.33 \\
		     & VP-IF &           93.14 $\pm$ 0.19 &           90.78 $\pm$ 0.22 &           93.33 $\pm$ 0.20 &           90.46 $\pm$ 0.43 &           84.00 $\pm$ 0.41 &  \textbf{71.69 $\pm$ 0.30} \\
		     & VP-B &  \textbf{93.44 $\pm$ 0.29} &  \textbf{91.11 $\pm$ 0.26} &  \textbf{94.18 $\pm$ 0.14} &  \textbf{93.65 $\pm$ 0.07} &  \textbf{87.47 $\pm$ 0.31} &           70.39 $\pm$ 0.24 \\
		\cline{1-8}
		\multirow{4}{*}{0.50} & VP &           89.98 $\pm$ 0.44 &           84.07 $\pm$ 0.93 &           93.14 $\pm$ 0.29 &           86.89 $\pm$ 0.37 &           86.71 $\pm$ 0.41 &           71.21 $\pm$ 0.23 \\
		     & VP-$A^3$ &           93.71 $\pm$ 0.51 &           92.17 $\pm$ 0.39 &           87.71 $\pm$ 1.25 &           92.06 $\pm$ 0.13 &           84.91 $\pm$ 0.26 &           72.87 $\pm$ 0.19 \\
		     & VP-IF &           93.81 $\pm$ 0.48 &           91.62 $\pm$ 0.42 &           93.64 $\pm$ 0.13 &           89.97 $\pm$ 0.39 &           84.54 $\pm$ 0.34 &  \textbf{73.84 $\pm$ 0.20} \\
		     & VP-B &  \textbf{94.29 $\pm$ 0.34} &  \textbf{92.21 $\pm$ 0.27} &  \textbf{94.41 $\pm$ 0.19} &  \textbf{93.70 $\pm$ 0.04} &  \textbf{88.09 $\pm$ 0.35} &           72.41 $\pm$ 0.11 \\
		\cline{1-8}
		\multirow{4}{*}{0.70} & VP &           92.51 $\pm$ 0.51 &           91.88 $\pm$ 0.25 &           94.26 $\pm$ 0.20 &           93.46 $\pm$ 0.10 &           88.12 $\pm$ 0.33 &           73.73 $\pm$ 0.19 \\
		     & VP-$A^3$ &           94.25 $\pm$ 0.43 &           94.23 $\pm$ 0.26 &           88.79 $\pm$ 1.45 &           92.58 $\pm$ 0.09 &           86.63 $\pm$ 0.28 &           73.34 $\pm$ 0.12 \\
		     & VP-IF &           94.50 $\pm$ 0.37 &           94.48 $\pm$ 0.24 &           93.94 $\pm$ 0.17 &           92.28 $\pm$ 0.10 &           86.40 $\pm$ 0.29 &  \textbf{74.66 $\pm$ 0.20} \\
		     & VP-B &  \textbf{94.92 $\pm$ 0.53} &  \textbf{94.87 $\pm$ 0.16} &  \textbf{94.46 $\pm$ 0.20} &  \textbf{94.03 $\pm$ 0.06} &  \textbf{88.70 $\pm$ 0.26} &           73.02 $\pm$ 0.09 \\
		\cline{1-8}
		\multirow{4}{*}{0.90} & VP &           95.08 $\pm$ 0.15 &           93.59 $\pm$ 0.22 &  \textbf{94.47 $\pm$ 0.15} &           93.61 $\pm$ 0.15 &  \textbf{89.07 $\pm$ 0.23} &  \textbf{75.43 $\pm$ 0.15} \\
		     & VP-$A^3$ &           95.62 $\pm$ 0.15 &           95.97 $\pm$ 0.11 &           90.91 $\pm$ 0.39 &           93.32 $\pm$ 0.14 &           88.67 $\pm$ 0.27 &           72.39 $\pm$ 0.11 \\
		     & VP-IF &  \textbf{95.91 $\pm$ 0.17} &           95.82 $\pm$ 0.13 &           94.40 $\pm$ 0.20 &           92.93 $\pm$ 0.11 &           88.82 $\pm$ 0.34 &           74.64 $\pm$ 0.13 \\
		     & VP-B &           95.57 $\pm$ 0.16 &  \textbf{96.02 $\pm$ 0.10} &           94.25 $\pm$ 0.24 &  \textbf{93.80 $\pm$ 0.19} &           88.79 $\pm$ 0.30 &           72.26 $\pm$ 0.27 \\
		\bottomrule
	\end{tabular}
}
\end{table}


==> standard-vae-pu/Precision.tex <==
\begin{table}[tbp]
	\centering \scriptsize \renewcommand{\arraystretch}{1.2}
	\caption{Precision values -- VAE-PU-Bayes (traditional PU setting)}
	\label{tab:Precision}
\scalebox{0.63}{
	\begin{tabular}{llllllll}
		\toprule
		\textbf{c} & \textbf{Method} & \textbf{MNIST 3v5} & \textbf{MNIST OvE} & \textbf{CIFAR CT} & \textbf{CIFAR MA} & \textbf{STL MA} & \textbf{CDC Diabetes} \\
		\midrule
		\multirow{4}{*}{0.02} & VP &           76.17 $\pm$ 0.67 &           65.82 $\pm$ 1.67 &           82.00 $\pm$ 0.70 &           83.53 $\pm$ 1.02 &           73.30 $\pm$ 0.55 &           50.44 $\pm$ 0.21 \\
		     & VP-$A^3$ &  \textbf{77.52 $\pm$ 0.63} &           72.40 $\pm$ 1.87 &           81.61 $\pm$ 1.34 &           84.81 $\pm$ 0.76 &           72.88 $\pm$ 0.88 &           52.72 $\pm$ 1.22 \\
		     & VP-IF &           77.31 $\pm$ 1.02 &  \textbf{77.70 $\pm$ 1.38} &           90.40 $\pm$ 1.59 &           87.14 $\pm$ 1.19 &           79.48 $\pm$ 2.68 &           51.58 $\pm$ 0.94 \\
		     & VP-B &           76.88 $\pm$ 0.84 &           73.90 $\pm$ 1.61 &  \textbf{91.72 $\pm$ 0.96} &  \textbf{91.94 $\pm$ 0.24} &  \textbf{82.14 $\pm$ 0.80} &  \textbf{58.07 $\pm$ 1.45} \\
		\cline{1-8}
		\multirow{4}{*}{0.10} & VP &           77.24 $\pm$ 0.70 &           69.92 $\pm$ 0.93 &           87.69 $\pm$ 0.30 &           84.77 $\pm$ 0.61 &           76.14 $\pm$ 0.46 &           50.72 $\pm$ 0.21 \\
		     & VP-$A^3$ &  \textbf{90.13 $\pm$ 0.39} &           81.84 $\pm$ 2.00 &           86.77 $\pm$ 0.94 &           87.23 $\pm$ 0.77 &           77.71 $\pm$ 0.63 &           57.60 $\pm$ 1.26 \\
		     & VP-IF &           90.11 $\pm$ 0.36 &           82.29 $\pm$ 1.80 &           91.02 $\pm$ 1.07 &           82.79 $\pm$ 1.14 &           82.49 $\pm$ 1.72 &           54.98 $\pm$ 1.16 \\
		     & VP-B &           90.08 $\pm$ 0.56 &  \textbf{84.06 $\pm$ 1.31} &  \textbf{93.97 $\pm$ 0.20} &  \textbf{92.39 $\pm$ 0.26} &  \textbf{85.05 $\pm$ 0.33} &  \textbf{63.76 $\pm$ 0.90} \\
		\cline{1-8}
		\multirow{4}{*}{0.30} & VP &           80.89 $\pm$ 0.58 &           76.61 $\pm$ 0.34 &           91.27 $\pm$ 0.44 &           89.16 $\pm$ 0.32 &           81.65 $\pm$ 0.44 &           52.31 $\pm$ 0.22 \\
		     & VP-$A^3$ &  \textbf{93.87 $\pm$ 0.26} &  \textbf{90.20 $\pm$ 0.37} &           87.88 $\pm$ 1.05 &           89.93 $\pm$ 0.48 &           80.03 $\pm$ 0.64 &           65.87 $\pm$ 0.54 \\
		     & VP-IF &           93.51 $\pm$ 0.31 &           89.98 $\pm$ 0.43 &           94.28 $\pm$ 0.52 &           86.78 $\pm$ 1.05 &           85.21 $\pm$ 1.74 &           63.92 $\pm$ 0.58 \\
		     & VP-B &           92.96 $\pm$ 0.37 &           89.85 $\pm$ 0.38 &  \textbf{94.88 $\pm$ 0.17} &  \textbf{93.73 $\pm$ 0.12} &  \textbf{88.00 $\pm$ 0.40} &  \textbf{69.23 $\pm$ 0.34} \\
		\cline{1-8}
		\multirow{4}{*}{0.50} & VP &           82.82 $\pm$ 0.70 &           73.22 $\pm$ 1.55 &           90.31 $\pm$ 0.54 &           77.99 $\pm$ 0.65 &           81.66 $\pm$ 1.05 &           56.12 $\pm$ 0.30 \\
		     & VP-$A^3$ &           93.87 $\pm$ 0.70 &           90.60 $\pm$ 0.66 &           89.32 $\pm$ 1.21 &           89.84 $\pm$ 0.30 &           82.23 $\pm$ 0.52 &           68.43 $\pm$ 0.30 \\
		     & VP-IF &           93.98 $\pm$ 0.62 &  \textbf{92.20 $\pm$ 0.38} &           95.29 $\pm$ 0.36 &           90.93 $\pm$ 1.17 &           88.00 $\pm$ 1.62 &           66.65 $\pm$ 0.33 \\
		     & VP-B &  \textbf{94.25 $\pm$ 0.33} &           91.95 $\pm$ 0.41 &  \textbf{95.33 $\pm$ 0.19} &  \textbf{94.03 $\pm$ 0.19} &  \textbf{89.43 $\pm$ 0.34} &  \textbf{70.90 $\pm$ 0.26} \\
		\cline{1-8}
		\multirow{4}{*}{0.70} & VP &           87.86 $\pm$ 0.65 &           85.94 $\pm$ 0.43 &           93.54 $\pm$ 0.29 &           91.49 $\pm$ 0.32 &           85.42 $\pm$ 0.69 &           60.00 $\pm$ 0.29 \\
		     & VP-$A^3$ &           94.63 $\pm$ 0.48 &           93.29 $\pm$ 0.43 &           89.40 $\pm$ 1.32 &           91.17 $\pm$ 0.30 &           85.29 $\pm$ 0.63 &           70.06 $\pm$ 0.23 \\
		     & VP-IF &  \textbf{95.46 $\pm$ 0.28} &           93.95 $\pm$ 0.37 &           94.88 $\pm$ 0.36 &           90.78 $\pm$ 0.43 &           88.72 $\pm$ 1.24 &           68.06 $\pm$ 0.26 \\
		     & VP-B &           94.82 $\pm$ 0.53 &  \textbf{94.21 $\pm$ 0.20} &  \textbf{95.35 $\pm$ 0.16} &  \textbf{94.69 $\pm$ 0.13} &  \textbf{89.61 $\pm$ 0.36} &  \textbf{71.50 $\pm$ 0.23} \\
		\cline{1-8}
		\multirow{4}{*}{0.90} & VP &           92.73 $\pm$ 0.22 &           88.86 $\pm$ 0.38 &           94.94 $\pm$ 0.28 &           91.71 $\pm$ 0.43 &           88.31 $\pm$ 0.48 &           65.49 $\pm$ 0.30 \\
		     & VP-$A^3$ &           95.72 $\pm$ 0.24 &           95.42 $\pm$ 0.04 &           93.10 $\pm$ 0.40 &           93.45 $\pm$ 0.19 &           89.95 $\pm$ 0.35 &           71.98 $\pm$ 0.27 \\
		     & VP-IF &  \textbf{97.10 $\pm$ 0.21} &  \textbf{96.50 $\pm$ 0.09} &  \textbf{95.91 $\pm$ 0.19} &  \textbf{96.88 $\pm$ 0.07} &  \textbf{91.74 $\pm$ 0.34} &           69.20 $\pm$ 0.38 \\
		     & VP-B &           95.62 $\pm$ 0.25 &           95.70 $\pm$ 0.15 &           95.00 $\pm$ 0.24 &           94.94 $\pm$ 0.12 &           90.58 $\pm$ 0.34 &  \textbf{72.12 $\pm$ 0.22} \\
		\bottomrule
	\end{tabular}
}
\end{table}


==> standard-vae-pu/Recall.tex <==
\begin{table}[tbp]
	\centering \scriptsize \renewcommand{\arraystretch}{1.2}
	\caption{Recall values -- VAE-PU-Bayes (traditional PU setting)}
	\label{tab:Recall}
\scalebox{0.63}{
	\begin{tabular}{llllllll}
		\toprule
		\textbf{c} & \textbf{Method} & \textbf{MNIST 3v5} & \textbf{MNIST OvE} & \textbf{CIFAR CT} & \textbf{CIFAR MA} & \textbf{STL MA} & \textbf{CDC Diabetes} \\
		\midrule
		\multirow{4}{*}{0.02} & VP &  \textbf{89.93 $\pm$ 0.94} &  \textbf{85.73 $\pm$ 0.82} &  \textbf{95.74 $\pm$ 0.55} &  \textbf{95.12 $\pm$ 0.24} &  \textbf{85.52 $\pm$ 1.18} &  \textbf{98.12 $\pm$ 0.29} \\
		     & VP-$A^3$ &           85.49 $\pm$ 0.86 &           82.40 $\pm$ 0.51 &           87.55 $\pm$ 1.06 &           93.63 $\pm$ 0.68 &           78.95 $\pm$ 0.57 &           87.83 $\pm$ 2.40 \\
		     & VP-IF &           86.59 $\pm$ 0.78 &           77.24 $\pm$ 1.33 &           89.97 $\pm$ 0.94 &           88.56 $\pm$ 1.15 &           71.01 $\pm$ 1.12 &           94.39 $\pm$ 1.87 \\
		     & VP-B &           85.74 $\pm$ 0.88 &           72.28 $\pm$ 1.92 &           91.81 $\pm$ 1.01 &           92.29 $\pm$ 0.26 &           79.12 $\pm$ 0.76 &           58.48 $\pm$ 0.99 \\
		\cline{1-8}
		\multirow{4}{*}{0.10} & VP &  \textbf{98.11 $\pm$ 0.25} &  \textbf{96.30 $\pm$ 0.27} &  \textbf{95.95 $\pm$ 0.30} &  \textbf{96.10 $\pm$ 0.16} &  \textbf{92.44 $\pm$ 0.32} &  \textbf{98.65 $\pm$ 0.14} \\
		     & VP-$A^3$ &           91.04 $\pm$ 0.36 &           86.40 $\pm$ 0.42 &           95.61 $\pm$ 0.42 &           94.75 $\pm$ 0.36 &           87.74 $\pm$ 0.50 &           79.37 $\pm$ 2.39 \\
		     & VP-IF &           91.51 $\pm$ 0.37 &           86.62 $\pm$ 0.52 &           94.22 $\pm$ 0.56 &           95.54 $\pm$ 0.33 &           82.79 $\pm$ 1.05 &           87.71 $\pm$ 2.35 \\
		     & VP-B &           92.88 $\pm$ 0.48 &           88.71 $\pm$ 0.56 &           93.47 $\pm$ 0.32 &           93.63 $\pm$ 0.18 &           86.41 $\pm$ 0.45 &           62.78 $\pm$ 0.79 \\
		\cline{1-8}
		\multirow{4}{*}{0.30} & VP &  \textbf{98.43 $\pm$ 0.21} &  \textbf{97.58 $\pm$ 0.10} &  \textbf{95.05 $\pm$ 0.22} &  \textbf{95.93 $\pm$ 0.10} &  \textbf{91.22 $\pm$ 0.41} &  \textbf{98.41 $\pm$ 0.09} \\
		     & VP-$A^3$ &           92.23 $\pm$ 0.33 &           91.11 $\pm$ 0.34 &           92.94 $\pm$ 1.02 &           94.15 $\pm$ 0.45 &           88.27 $\pm$ 0.38 &           76.28 $\pm$ 0.60 \\
		     & VP-IF &           92.81 $\pm$ 0.31 &           91.61 $\pm$ 0.31 &           92.45 $\pm$ 0.29 &           94.57 $\pm$ 0.44 &           83.72 $\pm$ 1.17 &           81.71 $\pm$ 0.59 \\
		     & VP-B &           93.93 $\pm$ 0.35 &           92.41 $\pm$ 0.15 &           93.50 $\pm$ 0.25 &           93.58 $\pm$ 0.09 &           86.96 $\pm$ 0.46 &           71.62 $\pm$ 0.41 \\
		\cline{1-8}
		\multirow{4}{*}{0.50} & VP &  \textbf{98.54 $\pm$ 0.21} &  \textbf{98.95 $\pm$ 0.22} &  \textbf{96.18 $\pm$ 0.29} &  \textbf{98.13 $\pm$ 0.10} &  \textbf{92.59 $\pm$ 0.68} &  \textbf{97.40 $\pm$ 0.10} \\
		     & VP-$A^3$ &           93.59 $\pm$ 0.45 &           93.81 $\pm$ 0.33 &           86.70 $\pm$ 2.02 &           94.41 $\pm$ 0.23 &           87.88 $\pm$ 0.59 &           77.94 $\pm$ 0.24 \\
		     & VP-IF &           93.66 $\pm$ 0.46 &           91.21 $\pm$ 0.93 &           92.09 $\pm$ 0.28 &           89.70 $\pm$ 1.44 &           82.29 $\pm$ 1.46 &           82.80 $\pm$ 0.34 \\
		     & VP-B &           94.34 $\pm$ 0.46 &           92.48 $\pm$ 0.29 &           93.51 $\pm$ 0.27 &           93.37 $\pm$ 0.18 &           86.79 $\pm$ 0.39 &           74.00 $\pm$ 0.32 \\
		\cline{1-8}
		\multirow{4}{*}{0.70} & VP &  \textbf{97.69 $\pm$ 0.44} &  \textbf{98.71 $\pm$ 0.07} &  \textbf{94.99 $\pm$ 0.17} &  \textbf{95.52 $\pm$ 0.21} &  \textbf{91.04 $\pm$ 0.45} &  \textbf{95.62 $\pm$ 0.16} \\
		     & VP-$A^3$ &           93.90 $\pm$ 0.52 &           95.21 $\pm$ 0.37 &           88.28 $\pm$ 1.71 &           94.05 $\pm$ 0.27 &           88.12 $\pm$ 0.46 &           76.95 $\pm$ 0.26 \\
		     & VP-IF &           93.60 $\pm$ 0.58 &           95.03 $\pm$ 0.33 &           93.04 $\pm$ 0.29 &           93.86 $\pm$ 0.34 &           84.69 $\pm$ 0.99 &           82.69 $\pm$ 0.38 \\
		     & VP-B &           95.04 $\pm$ 0.61 &           95.54 $\pm$ 0.15 &           93.58 $\pm$ 0.28 &           93.39 $\pm$ 0.10 &           87.81 $\pm$ 0.27 &           74.62 $\pm$ 0.22 \\
		\cline{1-8}
		\multirow{4}{*}{0.90} & VP &  \textbf{97.56 $\pm$ 0.11} &  \textbf{98.86 $\pm$ 0.06} &  \textbf{94.02 $\pm$ 0.29} &  \textbf{95.60 $\pm$ 0.17} &  \textbf{89.88 $\pm$ 0.36} &  \textbf{88.95 $\pm$ 0.28} \\
		     & VP-$A^3$ &           95.53 $\pm$ 0.32 &           96.53 $\pm$ 0.22 &           88.85 $\pm$ 0.58 &           93.20 $\pm$ 0.21 &           87.44 $\pm$ 0.42 &           72.82 $\pm$ 0.29 \\
		     & VP-IF &           94.75 $\pm$ 0.34 &           95.15 $\pm$ 0.23 &           92.95 $\pm$ 0.26 &           89.29 $\pm$ 0.20 &           86.09 $\pm$ 0.54 &           81.08 $\pm$ 0.62 \\
		     & VP-B &           95.52 $\pm$ 0.24 &           96.34 $\pm$ 0.14 &           93.51 $\pm$ 0.32 &           92.70 $\pm$ 0.38 &           87.08 $\pm$ 0.40 &           72.43 $\pm$ 0.60 \\
		\bottomrule
	\end{tabular}
}
\end{table}

